Near-optimal Anomaly Detection in Graphs using Lovasz Extended Scan Statistic

The detection of anomalous activity in graphs is a statistical problem that arises in many applications, such as network surveillance, disease outbreak detection, and activity monitoring in social networks. Beyond its wide applicability, graph structured anomaly detection serves as a case study in the difficulty of balancing computational complexity with statistical power. In this work, we develop from first principles the generalized likelihood ratio test for determining if there is a well connected region of activation over the vertices in the graph in Gaussian noise. Because this test is computationally infeasible, we provide a relaxation, called the Lovasz extended scan statistic (LESS) that uses submodularity to approximate the intractable generalized likelihood ratio. We demonstrate a connection between LESS and maximum a-posteriori inference in Markov random fields, which provides us with a poly-time algorithm for LESS. Using electrical network theory, we are able to control type 1 error for LESS and prove conditions under which LESS is risk consistent. Finally, we consider specific graph models, the torus, k-nearest neighbor graphs, and epsilon-random graphs. We show that on these graphs our results provide near-optimal performance by matching our results to known lower bounds.

==> detector.tex <==
\section{Graph Cut Detector}

The scan statistic framework will motivate our detector.
Consider testing the null hypothesis $H_0 = \{\Ncal(0,\sigma^2 \Ib_p)\}$ against the point alternative $H_1^C = \{ \Ncal( \frac{\mu}{\sqrt{|C|}} \one_C) \}$ for some $C \subset [p]$.
Then consider the test statistic, $Z_C = \one_C^\top \yb / \sqrt{|C|}$, with corresponding p-value, $\Phi (Z_C/\sigma)$, the survival function of the standard normal.
From these point hypotheses, we form the test for our composite alternative $H_1 = \cup_{C \in \Ccal} H_1^C$, given by the test statistic, 
\begin{equation}
\label{eq:scan_stat}
Z = \sup_{C \in \Ccal} Z_C = \sup_{C \in \Ccal} \frac{\one_C^\top \yb}{\sqrt{|C|}}
\end{equation}

\[
\begin{aligned}
\frac{\one_{\hat C}^\top}{\sqrt{|\hat C|}} \frac{\one_C}{\sqrt{|C|}} = \frac{\one_{\hat C}^\top}{\sqrt{|\hat C|}} \yb + \frac{\one_{\hat C}^\top}{\sqrt{|\hat C|}} \epsilonb
\end{aligned}
\]

\subsection{The Complexity of Graph Cuts}

Let $\xi \in \RR^n$ be a random variable distributed according to a product measure $\PP$.
Then the $\PP$-complexity of the class $\Ccal \subset 2^{[n]}$ is given by
\[
\Upsilon_{\PP}(\Ccal) = \EE_{\PP} \sup_{C \in \Ccal} \frac{\one_C^\top \xi}{\sqrt{|C|}}
\]
We will primarily consider the Gaussian and Rademacher complexity which we call $g(\Ccal)$ and $b(\Ccal)$ respectively.
We would like to answer the question, what is a good bound on either $g(\Ccal)$ or $b(\Ccal)$ where $\Ccal = \{C \subset [n] : |\partial C| \le \rho \}$?
Incidentally this will provide a bound on the $VC$ dimension of $\Ccal$.
The following is a simple bound based on the cut counting theorem of Karger.

\begin{proposition}
Let $d_{\min}$ denote the minimum degree of any edge in $E$.
\[
g(\Ccal) \le L \sqrt{\frac{\rho}{d_{\min}} \log(n)}
\]
where $L$ is some universal constant.
\end{proposition}

\begin{proof}
Let $N(\Ccal,\epsilon)$ be the $\epsilon$-covering number of $\Ccal$ where the distance between $C,C' \in \Ccal$ is given by $2(1 - \frac{|C \cap C'|}{\sqrt{|C||C'|}})$.
By Dudley's bound of the Gaussian complexity we know that because the diameter of $\Ccal$ is $2$ then
\[
g(\Ccal) \le L \int_0^\infty \sqrt{\log N(\Ccal,\epsilon)} d\epsilon \le 2 L \sqrt{\log |\Ccal|}
\]
where $L$ is some universal constant.
It is known by Karger's cut counting theorem that $|\Ccal| \le n^{2\rho/d_{\min}}$ from which the statement follows.
\end{proof}

Based on our lower bound we know then that up to log factors this is tight for a $d$-regular graph.
But using the UST we can provide a bound that is more robust to minor changes in the degree distribution, such as the creation of an vertex with degree $1$ (in which case this becomes the trivial bound).

\begin{theorem}

Let $r_e$ denote the effective resistance of $e$, $r_{\partial C} = \sum_{e \in \partial C} r_e$, and $r_\Ccal = \max \{ r_{\partial C} : C \in \Ccal \}$.
Suppose that $r_\Ccal \le n$ then
\[
g(\Ccal) \le 2 \left(\sqrt{r_\Ccal} + \sqrt{\frac{1}{2} \log n}\right)\sqrt{\log (n-1)} + 2 \sqrt{\log 2}
\]

\end{theorem}

\begin{proof}

Let $\Ccal(\Tcal) = \{C \subset [n] : \|\nabla_\Tcal \one_C \|_1 \le (\sqrt{r_\Ccal} + \sqrt{\log 1/\delta})^2 \}$ and $\delta > 0$ then under the UST for any $C$, $\PP_\Tcal \{C \notin \Ccal(\Tcal)\} \le \delta$.
\[
\begin{aligned}
\EE_\xi \sup_{C \in \Ccal} \frac{\xi^\top \one_C}{\sqrt{|C|}} = \EE_\xi \sup_{C \in \Ccal} \EE_\Tcal  \frac{\xi^\top \one_C}{\sqrt{|C|}} \left[ \one\{ C \in \Ccal(\Tcal) \} + \one\{ C \notin \Ccal(\Tcal) \} \right] \\
\le \EE_\xi \sup_{C \in \Ccal} \left[ \EE_\Tcal \one\{ C \in \Ccal(\Tcal) \} \sup_{C' \in \Ccal(\Tcal)}  \frac{\xi^\top \one_{C'}}{\sqrt{|C'|}}
+ \EE_\Tcal \one\{ C \notin \Ccal(\Tcal) \} \sup_{C' \in 2^{[n]}} \frac{\xi^\top \one_C'}{\sqrt{|C'|}} \right]\\
\le \EE_\xi \sup_{C \in \Ccal} \left[ \EE_\Tcal \sup_{C' \in \Ccal(\Tcal)}  \frac{\xi^\top \one_{C'}}{\sqrt{|C'|}}
+ \EE_\Tcal \one\{ C \notin \Ccal(\Tcal) \} \sup_{C' \in 2^{[n]}} \frac{\xi^\top \one_C'}{\sqrt{|C'|}} \right]\\
\le \EE_\xi  \left[ \EE_\Tcal \sup_{C' \in \Ccal(\Tcal)}  \frac{\xi^\top \one_{C'}}{\sqrt{|C'|}}
+ \sup_{C \in \Ccal} \PP_\Tcal \{ C \notin \Ccal(\Tcal) \} \sup_{C' \in 2^{[n]}} \frac{\xi^\top \one_C'}{\sqrt{|C'|}} \right]\\
\le \EE_\Tcal g(\Ccal(\Tcal)) + g(2^{[n]}) \sup_{C \in \Ccal} \PP_\Tcal \{ C \notin \Ccal(\Tcal) \} 
\end{aligned}
\]

For any $\Tcal$, $|\Ccal(\Tcal)| \le (n - 1)^{(\sqrt{r_\Ccal} + \sqrt{\log 1/\delta})^2}$.
By the same arguments as in the previous proposition, 
\[
g(\Ccal(\Tcal)) \le 2 \sqrt{(\sqrt{r_\Ccal} + \sqrt{\log 1/\delta})^2 \log (n-1)}
\]
Furthermore, $g(2^{[n]}) \le a \sqrt{n}$ where $a = 2 \sqrt{\log 2}$.
Setting $\delta = n^{-1/2}$ we have the following bound on the Gaussian complexity,
\[
g(\Ccal) \le 2 (\sqrt{r_\Ccal} + \sqrt{\frac{1}{2} \log n})\sqrt{\log (n-1)} + a
\]

\textbf{TODO}: Why is $|\Ccal(\Tcal)| \le (n-1) \ldots$? Not a big issue but where does $n-1$ come from when there are still $n$ vertices in the tree?

\end{proof}

\subsection{Relaxation}

Consider the following relaxation of the above program.
\[
\hat s = \max_{\xb \in [0,1]^p} \frac{\xb^\top \xi}{\sqrt{\one^\top \xb}} \textrm{ s.t. } \| \nabla \xb \|_1 \le \rho
\]
We will define the following edge incidence matrix weighted by the effective resistances of the edges:
\[
\nabla_{\Rcal,e} = r_e (\delta_{e^+} - \delta_{e^-})
\]
As in the previous theorem we will define for a given spanning tree $\Tcal$,
\[
\Xcal(\Tcal) = \{ \xb : \| \nabla_\Tcal \xb \|_1 \le (\sqrt{r_\Xcal} + \sqrt{\log (1 / \delta)})^2 \}
\]
where $r_\Xcal = \max{\| \nabla_\Rcal \xb \|_1 : x \in \Xcal}$.
We obtain the following theorem.
\begin{theorem}
Under the null hypothesis, $\xb = \zero$, the relaxed test statistic has the following bound
\[
\begin{aligned}
\hat s \le \frac{\log (2p / \delta)}{\sqrt{ \left(\sqrt{r_\Xcal} + \sqrt{\frac 12 \log n} \right)^2 \log p} } + 2 \sqrt{\left(\sqrt{r_\Xcal} + \sqrt{\frac 12 \log n} \right)^2 \log p} \\
+ \sqrt{2 p \log p} + \sqrt{2 \log 1 / \delta}
\end{aligned}
\]
with probability at least $1 - \delta$.
\end{theorem}

\begin{proof}
\[
\begin{aligned}
\hat s = \sup_{\xb \in \Xcal} \frac{\xi^\top \xb}{\sqrt{\one^\top \xb}} = \sup_{\xb \in \Xcal} \EE_\Tcal  \frac{\xi^\top \xb}{\sqrt{\one^\top \xb}} \left[ \one\{ \xb \in \Xcal(\Tcal) \} + \one\{ \xb \notin \Xcal(\Tcal) \} \right] \\
\le \sup_{\xb \in \Xcal} \left[ \EE_\Tcal \one\{ \xb \in \Xcal(\Tcal) \} \sup_{\xb' \in \Xcal(\Tcal)}  \frac{\xi^\top \xb'}{\sqrt{\one^\top \xb'}}
+ \EE_\Tcal \one\{ \xb \notin \Xcal(\Tcal) \} \sup_{\xb' \in [0,1]^p} \frac{\xi^\top \xb'}{\sqrt{\one^\top \xb'}} \right]\\
\le \sup_{\xb \in \Xcal} \left[ \EE_\Tcal \sup_{\xb' \in \Xcal(\Tcal)}  \frac{\xi^\top \xb'}{\sqrt{\one^\top \xb'}}
+ \EE_\Tcal \one\{ \xb \notin \Xcal(\Tcal) \} \sup_{\xb' \in [0,1]^p} \frac{\xi^\top \xb'}{\sqrt{\one^\top \xb'}} \right]\\
\le \EE_\Tcal \sup_{\xb \in \Xcal(\Tcal)}  \frac{\xi^\top \xb}{\sqrt{\one^\top \xb}}
+ \sup_{\xb \in \Xcal} \PP_\Tcal \{ \xb \notin \Xcal(\Tcal) \} \sup_{\xb' \in [0,1]^p} \frac{\xi^\top \xb'}{\sqrt{\one^\top \xb'}} \\
\end{aligned}
\]

\begin{claim}
\[
\EE_\xi \sup_{\xb' \in [0,1]^p} \frac{\xi^\top \xb'}{\sqrt{\one^\top \xb'}} \le \sqrt{2 p \log 2}
\]
\end{claim}

We will proceed to prove the above claim.  In words it follows from the fact that solutions to the program are integral by the generic chaining.
\[
\begin{aligned}
\EE_\xi \sup_{\xb' \in [0,1]^p} \frac{\xi^\top \xb'}{\sqrt{\one^\top \xb'}} = \EE_\xi \sup_{t \in [p]} \frac 1{\sqrt{t}} \sup_{\xb' \in [0,1]^p: \one^\top \xb \le t} \xi^\top \xb' \\
= \EE_\xi \sup_{t \in [p]} \frac 1{\sqrt{t}} \sup_{\xb' \in \{0,1\}^p: \one^\top \xb \le t} \xi^\top \xb' = \EE_\xi \sup_{\xb' \in \{0,1\}^p} \frac{\xi^\top \xb'}{\| \xb'\|} \le \sqrt{2 p \log 2}\\
\end{aligned}
\]

\begin{claim}
Denote $r = (\sqrt{r_\Xcal} + \sqrt{\frac 12 \log p} )^2$.
For any spanning tree $\Tcal$,
\[
\sup_{\xb \in \Xcal(\Tcal)}  \frac{\xi^\top \xb}{\sqrt{\one^\top \xb}} \le \frac{\log (p / 2\delta)}{\sqrt{r \log p} } + 2 \sqrt{r \log p}
\]
with probability at least $1 - \delta$ under $H_0$.
\end{claim}

This will follow from weak duality and a clever choice of dual parameters.
When parsing the following arguments it is beneficial to note that for $a,b > 0$, $\sup_{t \in \RR} a t - b t^2 = a^2 / (4b)$.
\[
\begin{aligned}
\sup_{\xb \in \Xcal(\Tcal)} \frac{\xi^\top \xb}{\sqrt{\one^\top \xb}} = \sup_{t \in [p]} \frac 1{\sqrt{t}} \sup_{\xb \in \Xcal(\Tcal), \one^\top \xb \le t}  \xi^\top \xb\\
= \sup_{t \in [p]} \frac 1{\sqrt{t}} \sup_{\xb \in [0,1]^p} \inf_{\eta \ge 0} \xi^\top \xb - \eta_0 \one^\top \xb - \eta_1 \|\nabla_\Tcal \xb \|_1 + \eta_0 t + \eta_1 r\\
\le \sup_{t \in [p]} \frac 1{\sqrt{t}} \sup_{\xb \in \{0,1\}^p} \xi^\top \xb - \one^\top \xb \sqrt{\frac{r}{t} \log p} - \|\nabla_\Tcal \xb \|_1 \sqrt{\frac{t}{r} \log p} + 2 \sqrt{rt \log p}\\
= \sup_{k \in [p]} \sup_{\xb \in \{0,1\}^p : \| \nabla_\Tcal \xb \|_0 = k} \sup_{t \in [p]} \frac{\xi^\top \xb}{\sqrt t} - \frac{\one^\top \xb}{t} \sqrt{r \log p} - k \sqrt{\frac{1}{r} \log p} + 2 \sqrt{r \log p}\\
\le \sup_{k \in [p]} \sup_{\xb \in \{0,1\}^p : \| \nabla_\Tcal \xb \|_0 = k} \frac{(\xi^\top \xb)^2}{4 \| \xb \|^2 \sqrt{r \log p}} - k \sqrt{\frac{1}{r} \log p} + 2 \sqrt{r \log p}\\
\end{aligned}
\]
We know that with probability at least $1 - \delta$ for all $k \in [p]$,
\[
\sup_{\xb \in \{0,1\}^p, \|\nabla_\Tcal \xb \|_0 = k} \left| \frac{\xi^\top \xb}{\| \xb \|} \right| \le \sqrt{2 k \log p} + \sqrt{2 \log (2p / \delta)}
\]
So we can bound the above,
\[
\begin{aligned}
\sup_{\xb \in \Xcal(\Tcal)}  \frac{\xi^\top \xb}{\sqrt{\one^\top \xb}} \le \sup_{k \in [p]} \frac{(\sqrt{2 k \log p} + \sqrt{2 \log (2p / \delta)})^2}{4 \sqrt{r \log p}} - k \sqrt{\frac{1}{r} \log p} + 2 \sqrt{r \log p}\\
\le \sup_{k \in [p]} \frac{\sqrt{k \log (2p / \delta)}}{\sqrt{r}} - \frac{k}{2} \sqrt{\frac{\log p}{r}} + \frac{\log(2p / \delta)}{2\sqrt{r \log p}} + 2 \sqrt{r \log p}\\ 
\le \frac{\log (2p / \delta)}{2 \sqrt{r \log p} } + \frac{\log(2p / \delta)}{2\sqrt{r \log p}} + 2 \sqrt{r \log p}\\ 
\le \frac{\log (2p / \delta)}{\sqrt{r \log p} } + 2 \sqrt{r \log p}\\ 
\end{aligned}
\]
Combining all of these results,
\[
\begin{aligned}
\hat s \le \frac{\log (2p / \delta)}{\sqrt{ \left(\sqrt{r_\Xcal} + \sqrt{\frac 12 \log n} \right)^2 \log p} } + 2 \sqrt{\left(\sqrt{r_\Xcal} + \sqrt{\frac 12 \log n} \right)^2 \log p} \\
+ \sqrt{2 p \log p} + \sqrt{2 \log 1 / \delta}
\end{aligned}
\]

\end{proof}


\subsection{Submodular Strong Duality}

\begin{lemma}
\label{lem:submod_convex}
Let $\{F_i\}_{i = 1}^k$ be submodular functions over $\{0,1\}^p$ and $\rhobb \in \RR^k$.
Consider the Primal linear integer program with submodular constraints, for fixed $\yb \in \RR^p$,
\begin{equation}
\label{eq:submod_primal}
\min_{\xb \in \{0,1\}^p}  \xb^\top \yb \textrm{\quad s.t. \quad} \forall i \in [k], F_i(\xb) \le \rho_i
\end{equation}
Suppose this is primal feasible,
then dual to this is the convex program
\begin{equation}
\label{eq:submod_dual}
\max_{\etab \in \RR_+^k, \sbb_i \in \RR^p, i \in [k]}  - \sum_{v \in [p]} (y_v + \sum_{i=1}^k \eta_i s_{i,v})_- - \sum_{i = 1}^k \eta_i \tilde f_i (\sbb_i) - \etab^\top \rhobb
\end{equation}
where $f_i$ is the Lov\'asz extension of $F_i$ and $\tilde f_i$ is its Fenchel conjugate over $[0,1]^p$.
Let $\{\sbb_i^*,\eta_i^*\}$ be optima for \eqref{eq:submod_dual}, then 
\[
\xb^* = \{\yb + \sum_{i=1}^k \eta^*_i \sbb^*_i \le 0\}
\]
is an optima for \eqref{eq:submod_primal}.
The objectives at these optima for \eqref{eq:submod_primal} and \eqref{eq:submod_dual} are equal (strong duality).
\end{lemma}

\begin{proof}
Let's begin by introducing Lagrangian parameters, so that \eqref{eq:submod_primal} is equal to,
\[
\min_{\xb \in \{0,1\}^p} \sup_{\etab \in \RR_+^k}  \xb^\top \yb + \sum_{i = 1}^k \eta_i (F_i(\xb) - \rho_i)
\]
We introduce a result from submodular optimization [Bach] that 
\[
F_i(\xb) = \sup_{\sbb \in \RR^p} \sbb^\top \xb - \tilde f_i (\sbb)
\]
Hence, \eqref{eq:submod_primal} is equal to,
\[
\begin{aligned}
&\min_{\xb \in \{0,1\}^p} \sup_{\etab \in \RR_+^k} \sup_{\sbb_i \in \RR^p, i \in [k]} \xb^\top \yb + \sum_{i = 1}^k \eta_i (\sbb_i^\top \xb - \tilde f_i (\sbb_i) - \rho_i) \\
&\ge \min_{\xb \in [0,1]^p} \sup_{\etab \in \RR_+^k} \sup_{\sbb_i \in \RR^p, i \in [k]} \xb^\top \yb + \sum_{i = 1}^k \eta_i (\sbb_i^\top \xb - \tilde f_i (\sbb_i) - \rho_i) \\
\end{aligned}
\]
as a convex relaxation of the hypercube.  We will now show that the relaxation attains optimum at integral values of $\xb$, hence the above inequality is an equality.
Define $\textrm{obj}(\etab, \{\sbb_i\}, \xb) = \xb^\top \yb + \sum_{i = 1}^k \eta_i (\sbb_i^\top \xb - \tilde f_i (\sbb_i) - \rho_i)$ and notice that it is concave in $\etab, \{\sbb_i\}$ and convex in $\xb$.
Also, the domain $[0,1]^p$ is bounded and each domain of obj is non-empty closed and convex.
\[
\begin{aligned}
&\min_{\xb \in [0,1]^p} \sup_{\etab \in \RR_+^k} \sup_{\sbb_i \in \RR^p, i \in [k]} \textrm{obj}(\etab, \{\sbb_i\}, \xb) \\
& = \sup_{\etab \in \RR_+^k} \min_{\xb \in [0,1]^p} \sup_{\sbb_i \in \RR^p, i \in [k]} \textrm{obj}(\etab, \{\sbb_i\}, \xb) \\
& = \sup_{\etab \in \RR_+^k} \sup_{\sbb_i \in \RR^p, i \in [k]} \min_{\xb \in [0,1]^p} \textrm{obj}(\etab, \{\sbb_i\}, \xb) \\
\end{aligned}
\]
Both of these equalities follow from a saddlepoint result in Rockafeller p.393 Cor 37.3.2.
The first equality depends also on the fact that $\sup_{\sbb_i \in \RR^p, i \in [k]} \textrm{obj}(\etab, \{\sbb_i\}, \xb)$ is affine in $\etab$, while it is convex in $\xb$ (because it is the pointwise maximum of affine functions).
The second equality follows from the fact that obj with $\etab$ fixed is concave in $\{\sbb_i\}$ and affine in $\xb$.
Now, we see that because $\textrm{obj}(\etab, \{\sbb_i\}, \xb)$ is linear over $\xb$ then its optimum is attained at
\[
\xb^*(\etab, \{\sbb_i\}) = \{\yb + \sum_{i=1}^k \eta_i \sbb_i \le 0\}
\]
and so $\xb^*(\etab, \{\sbb_i\}) \in \{0,1\}^p$.
Let then the optima be the triplet $(\etab^*, \{\sbb_i^*\}, \xb^*)$.
And so fixing $\xb^* = \xb^*(\etab^*, \{\sbb^*_i\})$
\[
\begin{aligned}
\textrm{obj}(\etab^*, \{\sbb^*_i\}, \xb^*) = \min_{\xb \in \{0,1\}^p} \sup_{\etab \in \RR_+^k} \sup_{\sbb_i \in \RR^p, i \in [k]} \textrm{obj}(\etab, \{\sbb_i\}, \xb) \\
= \sup_{\etab \in \RR_+^k} \sup_{\sbb_i \in \RR^p, i \in [k]} \textrm{obj}(\etab, \{\sbb_i\}, \xb^*) \ge \min_{\xb \in \{0,1\}^p} \sup_{\etab \in \RR_+^k} \sup_{\sbb_i \in \RR^p, i \in [k]} \textrm{obj}(\etab, \{\sbb_i\}, \xb^*)
\end{aligned}
\]
Hence, \eqref{eq:submod_primal} is equal to $\textrm{obj}(\etab^*, \{\sbb^*_i\}, \xb)$.
\end{proof}


\begin{theorem}
\label{thm:submod_duality}
Define the Lagrangian of the submodular program \eqref{eq:submod_primal}:
\[
g(\xb,\etab) = \xb^\top \yb + \sum_{i \in [k]} \eta_i (F_i(\xb) - \rho_i)
\]
Then given primal feasibility,
\[
\min_{\xb \in \{0, 1\}^p} \max_{\etab \in \RR_+^k} g(\xb,\etab) = \max_{\etab \in \RR_+^k} \min_{\xb \in \{0, 1\}^p} g(\xb,\etab)
\]
Moreover, the Lagrangian dual function
\[
\min_{\xb \in \{0, 1\}^p} g(\xb,\etab)
\]
is concave in $\etab$.
\end{theorem}

\begin{proof}
We have shown in Lemma \ref{lem:submod_convex} that 
\[
\min_{\xb \in \{0, 1\}^k} \max_{\etab \in \RR_+^k} g(\xb,\etab)
= - \left( \min_{\etab \in \RR_+^k, \sbb_i \in \RR^p, i \in [k]}  \sum_{v \in [p]} (y_v + \sum_{i=1}^k \eta_i s_{i,v})_- + \sum_{i = 1}^k \eta_i \tilde f_i (\sbb_i) + \etab^\top \rhobb \right)
\]
Let us isolate the part of the RHS that depends on $\{ \sbb_i \}$, and then evaluate the Fenchel conjugate.
\begin{equation}
\label{eq:srhs}
\begin{aligned}
&\min_{\sbb_i\in \RR^p} \sum_{v \in [p]} (y_v + \sum_{i=1}^k \eta_i s_{i,v})_- + \sum_{i = 1}^k \eta_i \tilde f_i (\sbb_i) \\
&= \min_{\sbb_i\in \RR^p} \max_{\tilde \sbb_i \in [0,1]^p} \sum_{v \in [p]} (y_v + \sum_{i=1}^k \eta_i s_{i,v})_- + \sum_{i = 1}^k \eta_i (\sbb_i^\top \tilde \sbb_i - f_i (\tilde \sbb_i))\\
&= \max_{\tilde \sbb_i \in [0,1]^p} \min_{\sbb_i\in \RR^p} \sum_{v \in [p]} (y_v + \sum_{i=1}^k \eta_i s_{i,v})_- + \sum_{i = 1}^k \eta_i (\sbb_i^\top \tilde \sbb_i - f_i (\tilde \sbb_i))
\end{aligned}
\end{equation}
This saddlepoint result follows from Rockafeller p.393 Cor 37.3.2, and the fact that the objective is concave in $\tilde \sbb$, convex in $\sbb$, the domains are non-empty closed convex, and $[0,1]^p$ is bounded. 
We can now evaluate the term that depends on $\{s_{i,v}\}_i$. 
\[
(y_v + \sum_{j=1}^k \eta_j s_{j,v})_- + \sum_{j = 1}^k \eta_j s_{j,v} \tilde s_{j,v} = \left\{ 
\begin{array}{ll}
- y_v + \sum_{j=1}^k \eta_j s_{j,v} (\tilde s_{j,v} - 1), & y_v + \sum_{j=1}^k \eta_j s_{j,v} \le 0\\
\sum_{j = 1}^k \eta_j s_{j,v} \tilde s_{j,v}, & y_v + \sum_{j=1}^k \eta_j s_{j,v} > 0
\end{array}\right.
\]
Let $\Ical = \{i \in [k] : \eta_i > 0 \}$ and suppose that $\Ical \ne \emptyset$.
The subgradient in $s_{i,v}$ for $i \in \Ical$ is given by 
\[
\left\{
\begin{array}{ll}
\{ \eta_i (\tilde s_{i,v} - 1)\}, & y_v + \sum_{j=1}^k \eta_j s_{j,v} < 0\\
\{ \eta_i \tilde s_{i,v} \}, & y_v + \sum_{j=1}^k \eta_j s_{j,v} > 0\\ [0pt]
[\eta_i (\tilde s_{i,v} - 1), \eta_i \tilde s_{i,v}] , & y_v + \sum_{j=1}^k \eta_j s_{j,v} = 0\\
\end{array} \right.
\]
Now we can see that if $\tilde s_{i,v} < 1$ for $i \in \Ical$ then the minimizer will satisfy $y_v + \sum_{j=1}^k \eta_j s_{j,v} \ge 0$, and if 
$\tilde s_{i,v} > 0$ for $i \in \Ical$ then the minimizer will satisfy $y_v + \sum_{j=1}^k \eta_j s_{j,v} \le 0$.
Suppose there exists an $i$ such that $\tilde s_{i,v} \in (0,1)$, then the minimizer will satisfy $y_v + \sum_{j=1}^k \eta_j s_{j,v} = 0$ and the relevant term in the objective is $\sum_{j} \eta_j s_{j,v} \tilde s_{j,v}$.
So unless the vector $(\eta_j \tilde s_{j,v})_j$ is normal to the plane $y_v + \sum_{j=1}^k \eta_j s_{j,v} = 0$, then this will be minimized at $-\infty$.
This only occurs when $\tilde s_{j,v}$ are equal for all $j \in \Ical$.
Hence, we are able to assume that either $\tilde s_{i,v} \in\{0, 1\}$ for all $i\in \Ical$, $\tilde s_{i,v}$ are all equal for $i \in \Ical$, or the objective is minimized at $-\infty$.

Suppose that $\tilde s_{i,v} \in\{0, 1\}$ for all $i \in \Ical$.
Now let us evaluate the term dependent on $\{s_{i,v}\}_i$, and let $A = \{\tilde s_{i,v} = 1\} \cap \Ical$.
\[
\left\{
\begin{array}{ll}
- y_v - \sum_{j \in \Ical \backslash A} \eta_j s_{j,v}, & y_v + \sum_{j=1}^k \eta_j s_{j,v} \le 0\\
\sum_{j \in A} \eta_j s_{j,v}, & y_v + \sum_{j=1}^k \eta_j s_{j,v} > 0
\end{array}\right.
\]
So as before, the minimizer will satisfy in both of these cases $y_v + \sum_{j=1}^k \eta_j s_{j,v} = 0$ or the minimum is $-\infty$.
This implies that $A = \Ical$ or $A = \emptyset$ with the objective above evaluating to $-y_v$ or $0$ respectively.
Combining these conclusions, we find that $\{ \tilde s_{i,v}\}_{i \in \Ical}$ must be identical, so we can introduce the variable $\tilde s_v$ and rewrite \eqref{eq:srhs} as
\[
\max_{\tilde \sbb \in [0,1]^p} -\yb^\top \tilde \sbb - \sum_{i = 1}^k \eta_i f_i(\tilde \sbb) = \max_{\tilde \sbb \in \{0,1\}^p} -\yb^\top \tilde \sbb - \sum_{i = 1}^k \eta_i f_i(\tilde \sbb)
\]
This follows from the fact that in \eqref{eq:srhs} only the set $\Ical$ contributes to the objective.
This follows from Prop 7 in [Bach], and the fact that $\yb^\top \tilde \sbb + \sum_{i = 1}^k \eta_i f_i(\tilde \sbb)$ is submodular.
\[
\min_{\xb \in \{0, 1\}^p} \max_{\etab \in \RR_+^k} g(\xb,\etab) = 
\max_{\etab \in \RR_+^k} - (\max_{\tilde \sbb \in \{0,1\}^p} - \yb^\top \tilde \sbb - \sum_{i = 1}^k \eta_i f_i(\tilde \sbb)) 
= \max_{\etab \in \RR_+^k} \min_{\xb \in \{0, 1\}^p} g(\xb,\etab)
\]
We know that the Lagrangian dual function
\[
\min_{\xb \in \{0, 1\}^p} g(\xb,\etab)
\]
is concave because it is the pointwise infimum of affine functions.
\end{proof}



\subsection{Low Cut Scan}

Perhaps the most well known inference procedure for noisy signals over graphs is maximum a-posteriori estimator (MAP) under a Markov random field (MRF).
We will focus on the binary label setting, in which there is an energy function that consists of a vertex potential and dyadic contributions,
\[
\min_{\xb \in \RR^p} \sum_{i \in V} \theta_i x_i + \sum_{i,j} w_{i,j} x_i x_j
\]
The MAP estimator for binary label noise under the Ising prior is known to take the form above.
Specifically, the problem above is solvable by graph cuts, which by the max flow - min cut duality, is solvable by max flow algorithms such as Ford-Fulkerson and Edmonds-Karp.
We will see that by Theorem \ref{thm:submod_duality}, this successive applications of cut problems will lead to an exact solution of the \eqref{eq:scan_stat}.

Notice that we can rewrite \eqref{eq:scan_stat} in the following way:
\[
\sup_{k \in [p]} \frac{1}{\sqrt{k}} \sup_{\xb \in \{0,1\}^p} \xb^\top \yb \textrm{ s.t. } \one^\top \xb \le k, \xb^\top \Delta \xb \le \rho  
\]
This follows from the fact that if $\xb$ is the minimizer for the inner program for $k$, and $\one^\top \xb < k$ then it is the minimizer for the inner program for $k \leftarrow k - 1$.
We will focus on solving the program,
\begin{equation}
\label{eq:inner_prog}
\sup_{\xb \in \{0,1\}^p} \xb^\top \yb \textrm{ s.t. } \one^\top \xb \le k, \xb^\top \Delta \xb \le \rho = - \sup_{\eta_0, \eta_1 \ge 0} \inf_{\xb \in \{0,1\}^p} g(\etab,\xb)
\end{equation}
where $g(\etab,\xb) = \yb^\top \xb + \eta_0 \one^\top \xb + \eta_1 \xb^\top \Delta \xb - \eta_0 k - \eta_1 \rho$.
Let us focus on solving the program,
\[
D(\etab) = \min_{\xb \in \{0,1\}^p} \yb^\top \xb + \eta_0 \one^\top \xb + \eta_1 \xb^\top \Delta \xb - \eta_0 k - \eta_1 \rho
\]
Because this is a minimum cut problem with an additional modular term, which is the same form as the MRF energy, this is solvable by graph cuts.
By the combinatorial duality of min cut this is equivalent to 
\[
M(\etab) = \max_{\fb \in \RR^{m + p}} \sum_{i \in [p]} f(s \rightarrow i) \textrm{ s.t. } \nabla^\top \fb = 0, \fb \le \cbb
\]
where $\nabla$ is the incidence matrix for the original graph $G$, the flow $\fb$ is over a modified graph with additional nodes $s,t$, and the capacitances are $c(i\rightarrow j) = \eta_1 w_{i,j}$ for $i,j$ in the graph, $c(s \rightarrow i) = (\eta_0 + y_i)_-$ and $c(i \rightarrow t) = (\eta_0 + y_i)_+$.
If in the final cut $i$ is connected to $s$ then $x_i = 1$ and $0$ otherwise.
Specifically, the Lagrangian dual is equal to 
\[
D(\etab) = - \sum_{i \in [p]} (y_i)_- + M(\etab) - \eta_0 k - \eta_1 \rho
\]
We can thus using residual flows ascertain the instantaneous effect of changing $\etab$ and thus compute gradients of the concave function $M(\etab)$.

Let us decompose the edges in the modified graph into $E_s, E_t, E$ the edges adjacent to $s$, $t$, and those of the original graph respectively.
Suppose that a flow $\fb^\star$ is the maximizer of $M(\etab)$, then let $B$ be the edges such that the flow equals the capacitance in the modified graph.
In the case that $B \subseteq E$ then we can change $\eta_1$ to $\eta_1'$ (as long as $\eta_1'$ is close enough to $\eta_1$) and then $\fb^\star$ may change to $\frac{\eta_1'}{\eta_1} \fb^\star = \eta_1' \Wb_B$ and the resulting flow is the maximizer of $M(\etab)$.
If on the other hand there are edges adjacent to $s$ or $t$ in $B$ then we must consider the following.
Let $\sum_{s\rightarrow i \in B} f^\star(s \rightarrow i) = \textrm{cflow}(s) = \sum_{s\rightarrow i \in B} (\eta_0 + y_i)_-$ and $\sum_{i\rightarrow t \in B} f^\star(i \rightarrow t) = \textrm{cflow}(t) = \sum_{i\rightarrow t \in B} (\eta_0 + y_i)_+$, then if $\eta_0$ is changed by a small enough amount (to $\eta_0'$), the flow is equal to the minimum of $\sum_{i\rightarrow t \in B} (\eta_0' + y_i)_-$ and $\sum_{s\rightarrow i \in B} (\eta_0 + y_i)_+$.
Hence, if $\textrm{cflow}(s) < \textrm{cflow}(t)$ then a change in $\eta_0$ by $\partial \eta_0$ would result in a change in $M(\etab)$ by $-|B \cap E_s| \partial \eta_0$, and if $\textrm{cflow}(s) > \textrm{cflow}(t)$ the same change would result in a change in $M(\etab)$ by $|B \cap E_t| \partial \eta_0$.
In the case of equality then the change would be the difference $(|B \cap E_t| - |B \cap E_s|) \partial \eta_0$.



